Query-Based Abstractive Summarization Using Neural Networks

In this paper, we present a model for generating summaries of text documents with respect to a query. This is known as query-based summarization. We adapt an existing dataset of news article summaries for the task and train a pointer-generator model using this dataset. The generated summaries are evaluated by measuring similarity to reference summaries. Our results show that a neural network summarization model, similar to existing neural network models for abstractive summarization, can be constructed to make use of queries to produce targeted summaries.

==> include/Acknowledgements.tex <==
\section*{Acknowledgments}
The acknowledgments should go immediately before the references.  Do
not number the acknowledgments section. Do not include this section
when submitting your paper for review.

==> include/settings/Settings.tex <==
% =======================
% COMPILE OPTIONS
% =======================

% Not important: Create if's for all options
\newif\ifunusedinbib
\newif\ifprintexamples
\newif\ifprintplannotes
\newif\iffixquotes
\newif\ifcolortext

% For each option below, comment out line ending with "true" to disable

% -----------------------
% Show unused references in bibliography
% Only enabled for checking if format looks correct for newly
% entered sources
% -----------------------
%\unusedinbibtrue

% -----------------------
% Automatically use correct start and end quotation character.
% Added as an option since not ending quotes give compile error,
% probably better to possible fix all at once
% -----------------------
\fixquotestrue


% =======================
% ENCODING
% =======================
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
%\pdfcompresslevel0

% =======================
% TEXT MACROS
% =======================

% Minimize macros
\newcommand{\nc}{\newcommand}

% =======================
% LANGUAGE
% =======================
\usepackage[english]{babel} % Language settings, last one will be primary language
\usepackage[utf8]{inputenc} % Input settings

% =======================
% MISC. PACKAGES
% =======================

% xcolor needs to be loaded earlier due to different arguments
\usepackage[usenames,dvipsnames]{xcolor}

%\usepackage{moreverb}                % List settings
% \usepackage{textcomp}               % Fonts, symbols etc.
% \usepackage{lmodern}                % Latin modern font
% \usepackage{helvet}                 % Enables font switching
\usepackage{amsmath}                % Mathematical expressions (American mathematical society)
\usepackage{amssymb}                % Mathematical symbols (American mathematical society)
% \usepackage{gensymb}
% \usepackage{graphicx}               % Figures
\usepackage{tabularx}
%\usepackage{ltablex} % Make tabularx split over pages?

% \usepackage{tabulary}
%\numberwithin{equation}{chapter}         % Numbering order for equations
%\numberwithin{figure}{chapter}           % Numbering order for figures
%\numberwithin{table}{chapter}            % Numbering order for tables
\usepackage{eso-pic}                % Create cover page background
%\usepackage{tikz}
%\usetikzlibrary{arrows,automata}
\usepackage{pgfplots}
\pgfplotsset{compat=1.13}
%\usepgflibrary{arrows}% for more options on arrows
%\usepackage[parfill]{parskip} % Vertical spacing between paragraphs, not first line indentation
%\usepackage{float}
%\usepackage{enumitem}
\usepackage{etoolbox}
%\usepackage{xifthen}
%\usepackage{enumitem}% http://ctan.org/pkg/enumitem

% Activate clickable links in table of contents 
%\usepackage[hidelinks]{hyperref}

%\usepackage{cleveref}
%\usepackage{comment}
%\usepackage{adjustbox}
%\usepackage{epigraph}
%\usepackage{setspace}

% Comment out to disable automatic hyphenation
%\usepackage[none]{hyphenat}

%\usepackage{multirow}
%\usepackage{mdframed}
%\usepackage{breqn}
% \usepackage[compact]{titlesec} % Compact titles
%\usepackage{scrextend}
%\usepackage{sectsty}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{setspace}
\usepackage{xspace}

%\usepackage[usenames,dvipsnames]{pstricks}
%\usepackage{epsfig}
%\usepackage{pst-grad} % For gradients
%\usepackage{pst-plot} % For axes
%\usepackage{tkz-graph}

% Force footnotes to bottom of page
\usepackage[bottom]{footmisc}

\usepackage{authblk}

\definecolor{Comment}{RGB}{255,255,224} %HELLO
\usepackage[
color=Comment,
linecolor=Red,
textsize=tiny,
%disable,
]{todonotes}
\newcommand{\todoinl}[1]{\todo[inline]{#1}}

% =======================
% CUSTOM ENVIRONMENTS AND MACROS
% =======================

% Custom commands and environments

\ifcolortext
\newcommand\mycolor[2][]{
\ifthenelse{\isempty{#1}}{\color{#2}}{\color[#1]{#2}}}
\else
\newcommand\mycolor[2][]{}
\fi

\newenvironment{draftenv}{\mycolor[RGB]{31,82,0}}{} % Green
\newenvironment{proposalenv}{\mycolor{Blue}}{}

\newcount\draftlevel
\draftlevel 4\relax

\def\draft{\begin{draftenv}}
\def\enddraft{\end{draftenv}}

\def\proposal{\begin{proposalenv}}
\def\endproposal{\end{proposalenv}}

% planningnote depend on setting
\ifprintplannotes
    \def\plannote{\bgroup\mycolor{Mahogany}}
    \def\endplannote{\egroup}
\else
    \let\plannote=\iffalse
    \let\endplannote=\fi
\fi

\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}

% C# with formatting
\newcommand{\CS}{C\texttt{\#}}

% Command for fancy R,as in real number set
\newcommand{\R}{\mathbb{R}}

% Citation missing command
\newcommand{\needcite}{\plannote\textbf{[citation~needed]}\endplannote}

% Looks better in phone numbers than standard + and -
\def\Plus{\texttt{+}}
\def\Minus{\texttt{-}}

% Concise way to make simple lists. The list spacing is changed in a pretty ugly way, differently for with and without argument.
\usepackage[sharp]{easylist}
\AtBeginEnvironment{easylist}{\ListProperties(Space=0cm, Space*=-0.08cm)}
\newenvironment{bulletlist}
{
    \begin{easylist}[itemize]
    \ListProperties(Space=0cm, Space*=-0.08cm)
}
{
    \end{easylist}
}

\newenvironment{numberedlist}
{
    \begin{easylist}[enumerate]
    \ListProperties(Space=0cm, Space*=-0.08cm)
}
{
    \end{easylist}
}

% =======================
% TEXT FORMATTING
% =======================

% Smart quotes
\usepackage[
  autostyle=false,
  english=american % Gives " ' ' " rather than British ' " " '
]{csquotes} % Smart quotation marks
\iffixquotes
\MakeOuterQuote{"}
%\MakeInnerQuote{'} % Not allowed since ' is reserved...
\fi

% =======================
% REFERENCE STUFF
% =======================
% References
\usepackage[
backend=biber, % 'biber' is a more modern backend, 'bibtex' is older alternative
%
% 'authoryear' give sort of what we've used before, 'numeric' is more like Wikipedia 
%style=numeric,
%style=numeric,
style=authoryear,
%style=apa,
%style=ieee,
%
%sorting=none, % 'none' gives order mentioned, 'ynt' is default
%autocite=footnote, % can be 'footnote', gives good results with 'authoryear'
maxbibnames=99,
mincitenames=1,
maxcitenames=2,
%maxnames=2,
urldate=iso8601,
%firstinits=true,
%uniquename=init
uniquelist=false
]{biblatex}
%\DeclareLanguageMapping{english}{english-apa}
\renewcommand*{\nameyeardelim}{\addcomma\space}
\renewcommand\cite{\autocite}

%\DeclareNameFormat{first-last}{%
        %\ifthenelse{\value{listcount}=1}
                %{
                %        \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
                %        \usebibmacro{name:andothers}
                %} 
                %{
                %        \ifthenelse{\value{listcount}>1\and\value{listtotal}>\value{liststop}}
                %        {}
                %        {%
                %            \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
                %        }%
                %}
%}

% Square brackets instead of parenthesis
%\makeatletter
%\newrobustcmd*{\parentexttrack}[1]{%
%	\begingroup%
%	\blx@blxinit%
%	\blx@setsfcodes%
%	\blx@bibopenparen#1\blx@bibcloseparen%
%	\endgroup}%
%\AtEveryCite{%
%	\let\parentext=\parentexttrack%
%	\let\bibopenparen=\bibopenbracket%
%	\let\bibcloseparen=\bibclosebracket}%
%\makeatother

%\usepackage[authordate,bibencoding=auto,strict,backend=biber,natbib]{biblatex-chicago}
% Hack to prevent replacing repeated author name with ------
%\renewbibmacro*{bbx:savehash}{}

\addbibresource{references.bib}

% Remove URL from academic articles (we still keep for @online sources)
% \AtEveryBibitem{%
% \ifentrytype{article}{
%     \clearfield{url}%
% 	\clearfield{urldate}%
%     \clearfield{urlyear}%
% }{}
% \ifentrytype{inproceedings}{
%     \clearfield{url}%
% 	\clearfield{urldate}%
%     \clearfield{urlyear}%
% }{}
% \ifentrytype{book}{
%     \clearfield{url}%
% 	\clearfield{urldate}%
%     \clearfield{urlyear}%
% }{}
% \ifentrytype{collection}{
%     \clearfield{url}%
% 	\clearfield{urldate}%
%     \clearfield{urlyear}%
% }{}
% \ifentrytype{incollection}{
%     \clearfield{url}%
% 	\clearfield{urldate}%
%     \clearfield{urlyear}%
% }{}
% }

% Remove URL from academic articles (we still keep for @online sources)
\AtEveryBibitem{%
\ifentrytype{online}{}{%
    \clearfield{url}%
	\clearfield{urldate}%
    \clearfield{urlyear}%
    }
}

% Never show DOI or ISBN, from Damaschke's comments
\AtEveryBibitem{%
    \clearfield{isbn}%
    \clearfield{issn}%
    \clearfield{doi}%
}

\setlength{\bibitemsep}{0.3cm}

%\DefineBibliographyStrings{english}{urlseen = {retrieved}}

% ============================
% CODE ENVIRONMENT
%============================
\usepackage{listings}               % Enables source code listings

% Different monospace font
\usepackage{inconsolata}

% Look of source code listing
\lstdefinestyle{mystyle}
{
    %backgroundcolor=,   
    %commentstyle=,
    %keywordstyle=,
    %numberstyle=,
    %stringstyle=,
    basicstyle=\footnotesize\ttfamily,
    %breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    %keepspaces=true,                 
    %numbers=left,                    
    %numbersep=5pt,                  
    %showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=4,
    frame = single,
    xleftmargin=0.8cm,
    xrightmargin=0.8cm,
    aboveskip=0.5cm,
    belowskip=0.5cm,
    extendedchars=false,
    inputencoding=utf8,
    %numbers=left
}
\lstset{style=mystyle}

\lstnewenvironment{algorithm}[1][] %defines the algorithm listing environment
{   
	%\captionsetup{labelformat=algocaption,labelsep=colon} %defines the caption setup for: it ises label format as the declared caption label above and makes label and caption text to be separated by a ':'
	\lstset{ %this is the stype
		mathescape=true,
		frame=single,
		numbers=left, 
		numberstyle=\small,
		basicstyle=\small, 
		keywordstyle=\color{black}\bfseries\em,
		%keywords={,input, output, return, datatype, function, in, if, else, foreach, while, begin, end, } %add the keywords you want, or load a language as Rubens explains in his comment above.
		numbers=left,
		columns=flexible,
        literate = {-}{-}1, % <------ trick!
		xleftmargin=.04\textwidth,
		#1 % this is to add specific settings to an usage of this environment (for instnce, the caption and referable label)
	}
}
{}

% Custom environment, for handling page breaks, see examples chapter
\lstnewenvironment{figcode}[2][]%
{%
  \lstset%
  {%
      style=mystyle,
      caption=#1,
      label=#2
  }%
  \noindent\minipage{\linewidth}%
}
{%
  \noindent\endminipage%
}


\lstnewenvironment{code}%
{%
  \lstset%
  {%
      style=mystyle,
  }%
  \noindent\minipage{\linewidth}%
}
{%
  \noindent\endminipage%
}

% Same, but with C# highlighting
\lstnewenvironment{figcscode}[2][]%
{%
  \lstset
  {%
      style=mystyle,
      caption=#1,
      label=#2,
      language=[Sharp]C,
      morekeywords={var}
  }%
  \noindent\minipage{\linewidth}%
}
{%
  \noindent\endminipage%
}

% Same, but with C# highlighting
\lstnewenvironment{cscode}%
{%
  \lstset
  {%
      style=mystyle,
      language=[Sharp]C,
      morekeywords={var}
  }%
  \noindent\minipage{\linewidth}%
}
{%
  \noindent\endminipage%
}

% =======================
% GENERAL DOCUMENT FORMATTING
% =======================

% Page style
% \usepackage[top=4cm, bottom=4cm,
%       inner=3.7cm, outer=3.7cm]{geometry}     % Page margin lengths

% Disable automatic indentation (equal to using \noindent)
%\setlength{\parindent}{0cm}                         

% Adjust table of contents spacing
%\usepackage[titles]{tocloft}

% Caption settings (aligned left with bold name)
\usepackage[labelfont=bf, textfont=normal,
      justification=justified,
      singlelinecheck=false,
      margin=0.5cm]{caption}  
% \usepackage[margin=0.2cm]{subcaption}
% \captionsetup{compatibility=false}

% BEWARE: ENABLING THIS MIGHT CHANGE SPACING SIGNIFICANTLY THROUGHOUT THE DOCUMENT
\usepackage[activate={true,nocompatibility},final,tracking=true,protrusion=false]{microtype}
% activate={true,nocompatibility} - activate protrusion and expansion
% final - enable microtype; use "draft" to disable
% tracking=true, kerning=true, spacing=true - activate these techniques
% factor=1100 - add 10% to the protrusion amount (default is 1000)
% stretch=10, shrink=10 - reduce stretchability/shrinkability (default is 20/20) 

% ================================
% Master thesis template settings
% ================================

% CREATED BY DAVID FRISK, 2016

% BASIC SETTINGS
\usepackage{moreverb}								% List settings
\usepackage{textcomp}								% Fonts, symbols etc.
\usepackage{lmodern}								% Latin modern font
\usepackage{helvet}									% Enables font switching
\usepackage{amsmath}								% Mathematical expressions (American mathematical society)
\usepackage{amssymb}								% Mathematical symbols (American mathematical society)
\usepackage{graphicx}								% Figures
%\usepackage{subfig}									% Enables subfigures
\numberwithin{equation}{chapter}					% Numbering order for equations
\numberwithin{figure}{chapter}						% Numbering order for figures
\numberwithin{table}{chapter}						% Numbering order for tables
\usepackage{listings}								% Enables source code listings
\usepackage{chemfig}								% Chemical structures
\usepackage[top=3cm, bottom=3cm,
			inner=3cm, outer=3cm]{geometry}			% Page margin lengths			
\usepackage{eso-pic}								% Create cover page background
\newcommand{\backgroundpic}[3]{
	\put(#1,#2){
	\parbox[b][\paperheight]{\paperwidth}{
	\centering
	\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
\usepackage{float} 									% Enables object position enforcement using [H]
\usepackage{parskip}								% Enables vertical spaces correctly 



% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)

% Disable automatic indentation (equal to using \noindent)
%\setlength{\parindent}{5cm}                         
%\setlength{\parskip}{5em}

%\usepackage[parfill]{parskip} % Vertical spacing between paragraphs, not first line indentation


% Caption settings (aligned left with bold name)
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{caption} 		

		  	
% Activate clickable links in table of contents  	
\usepackage{hyperxmp}
\usepackage{hyperref}						
\hypersetup{
colorlinks,
citecolor=black,
filecolor=black,
linkcolor=black,
urlcolor=black,
pdfauthor={Johan Hasselqvist, Niklas Helmertz, Mikael Kågebäck},
pdftitle={\mytitle},
pdfsubject={},
pdfkeywords={},
pdfproducer={},
pdfcreator={}
}

% Remove some additional pdf metadata
\ifdefined\pdftrailerid
\pdftrailerid{}
\fi

\ifdefined\pdfsuppressptexinfo
\pdfsuppressptexinfo15
\fi

% Define the number of section levels to be included in the t.o.c. and numbered	(3 is default)	
\setcounter{tocdepth}{5}							
\setcounter{secnumdepth}{6}	


% Chapter title settings
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]

% Header and footer settings (Select TWOSIDE or ONESIDE layout below)
\usepackage{fancyhdr}								
\pagestyle{fancy}  
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\space#1}{}} 


% Select one-sided (1) or two-sided (2) page numbering
\def\layout{1}	% Choose 1 for one-sided or 2 for two-sided layout

% Conditional expression based on the layout choice
\ifnum\layout=2	% Two-sided
    \fancyhf{}			 						
	\fancyhead[LE,RO]{\nouppercase{ \leftmark}}
	\fancyfoot[LE,RO]{\thepage}
	\fancypagestyle{plain}{			% Redefine the plain page style
	\fancyhf{}
	\renewcommand{\headrulewidth}{0pt} 		
	\fancyfoot[LE,RO]{\thepage}}	
\else			% One-sided  	
  	\fancyhf{}					
	\fancyhead[C]{\nouppercase{ \leftmark}}
	\fancyfoot[C]{\thepage}
\fi


% Enable To-do notes
%\usepackage[textsize=tiny]{todonotes}   % Include the option "disable" to hide all notes
\setlength{\marginparwidth}{2.5cm} 


% Supress warning from Texmaker about headheight
\setlength{\headheight}{15pt}		

